Face2QR: A Unified Framework for Aesthetic, Face-Preserving, and Scannable QR Code Generation

Existing methods to generate aesthetic QR codes, such as image and style transfer techniques, tend to compromise either the visual appeal or the scannability of QR codes when they incorporate human face identity. Addressing these imperfections, we present Face2QR-a novel pipeline specifically designed for generating personalized QR codes that harmoniously blend aesthetics, face identity, and scannability. Our pipeline introduces three innovative components. First, the ID-refined QR integration (IDQR) seamlessly intertwines the background styling with face ID, utilizing a unified Stable Diffusion (SD)-based framework with control networks. Second, the ID-aware QR ReShuffle (IDRS) effectively rectifies the conflicts between face IDs and QR patterns, rearranging QR modules to maintain the integrity of facial features without compromising scannability. Lastly, the ID-preserved Scannability Enhancement (IDSE) markedly boosts scanning robustness through latent code optimization, striking a delicate balance between face ID, aesthetic quality and QR functionality. In comprehensive experiments, Face2QR demonstrates remarkable performance, outperforming existing approaches, particularly in preserving facial recognition features within custom QR code designs. Codes are available at $\href{https://github.com/cavosamir/Face2QR}{\text{this URL link}}$.

==> sec/3_preliminaries.tex <==
\section{Preliminaries}
The tolerance of error is related to both the functional region and the information region. The marker and alignment pattern in functional region helps decoders to locate and decode information in the right sequence. Message is encoded in the information region with Reed–Solomon error correction codes~\cite{reed1960polynomial}. The encoding is in binary and usually represented by black and white modules (white for 1, black for 0). When decoding a QR code image $I$, the decoder will first transfer the image to a grayscale image by extracting the luminance channel. Two thresholds $\mathcal{T}_w=L\cdot(1+\alpha)/2$ and $\mathcal{T}_b=L\cdot(1-\alpha)/2$ are then used to generate binarized codes, with parameter $\alpha\in[0,1]$ deciding the strictness of binarization process. Let the width and height of the grayscale image be $W$ and $H$ pixels respectively. %, and the $p_i$ be pixel in the image, with coordinate $\mathbf{u}\in \{1, \ldots, W\}\times \{1, \ldots, H\}$. The binarization process can be described as:
For pixel $I(\mathbf{u})$ with coordinate $\mathbf{u}\in \{1, \ldots, W\}\times \{1, \ldots, H\}$, the binarization process can be described as:
\begin{gather}
    I^b(\mathbf{u}) = 
    \begin{cases}
        0, & \text{if } I^l(\mathbf{u}) < \mathcal{T}_b, \\
        1, & \text{if } I^l(\mathbf{u}) > \mathcal{T}_w, 
    \end{cases}
    % \mathcal{M}^r = \mathcal{E}_{r}(\mathcal{M}, I^{bin}).
\end{gather}
It is possible to have pixels with indefinite value when $\mathcal{T}_b \neq \mathcal{T}_w$.
After binarization, the decoder will try to find markers which have a black and white pattern of "1:1:3:1:1" ~\cite{zxing,antfu}. The decoder then locates the QR code and determines the module size $a$ according to the markers found, and create a grid that divides the image in to $n\times n$ modules each with size of $a\times a$. Then, the information is decoded module by module.
% Let the module coordinate in the image be $j \in \{1, \ldots, n\}\times \{1, \ldots, n\}$, and the decoder sensitive square area $\theta$ in the middle of each module be $b \times b$ in size. The averaging function for middle area is defined as
% \begin{equation}
%     avg(I^l_{QR}(j)) = \frac{1}{b^2}\sum_{i\in\theta}I^l_{QR}(i)
% \end{equation}
% Then, the information $E$ are decoded module by module.
% \begin{gather}
%     E(j) = 
%     \begin{cases}
%         0, & \text{if } avg(I^l_QR(j)) < \mathcal{T}_b, \\
%         1, & \text{if } avg(I^l_QR(j) > \mathcal{T}_w, 
%     \end{cases}
%     % \mathcal{M}^r = \mathcal{E}_{r}(\mathcal{M}, I^{bin}).
% \end{gather}

% \todo{QR code standard/decoding (maybe link to related previous work)}


==> sec/rebuttal.tex <==
\newpage
\clearpage
\renewcommand{\thetable}{\Alph{table}}
\newgeometry{left=4cm,right=4cm,top=2.6cm,bottom=2.cm}
% \newgeometry{top=2.5cm,bottom=2.5cm}
\setcounter{page}{1}
% \appendix

\vspace{-1pt}
\begin{table*}[ht]
    \newlength{\angles}
    \setlength{\angles}{0.156\textwidth}
    \vspace{-5pt}
    \centering
    \begin{minipage}[b]{.49\linewidth}
        \caption{Visual comparison with InstantID [38].}
        \vspace{-5pt}
        \label{tab:angle}
        \centering
        \begin{tabularx}{\linewidth}{>{\centering\arraybackslash}X *{3}{>{\centering\arraybackslash}X}}
    
        \toprule
        Input 
        &  InstantID & Face2QR \\
        \midrule
    
        % \includegraphics[width=\angles, height=\angles]{figures/lyf/lyf-90.png} & 
        % \includegraphics[width=\angles, height=\angles]{figures/lyf/outf0.5_1.0_15.0_new_doubleControl_54a27r11_0.80.81.4_300_00.png} & 
        % \includegraphics[width=\angles, height=\angles]{figures/lyf/outf0.5_1.0_15.0_new_doubleControl_54a27r11_0.80.81.4_300_00.png} \\
    
        % \includegraphics[width=\angles, height=\angles]{figures/lyf/lyf-45_1.png} & 
        % \includegraphics[width=\angles, height=\angles]{figures/lyf/outf0.5_1.0_15.0_new_doubleControl_53a27r11_0.80.81.4_300_00.png} & 
        % \includegraphics[width=\angles, height=\angles]{figures/lyf/outf0.5_1.0_15.0_new_doubleControl_53a27r11_0.80.81.4_300_00.png} \\

        \includegraphics[width=\angles, height=\angles]{figures/rebuttal/origin/zre_7.jpg} & 
        \includegraphics[width=\angles, height=\angles]{figures/rebuttal/inst/doubleControl_ZREIR7a4r17_0.80.81.4.png} & 
        \includegraphics[width=\angles, height=\angles]{figures/rebuttal/inst/outf1.5_1.0_15.0_doubleControl_ZRE7a4r17_0.80.81.4_200_00-100.png} \\
    
        \includegraphics[width=\angles, height=\angles]{figures/rebuttal/origin/zre_25.jpg} & 
        \includegraphics[width=\angles, height=\angles]{figures/rebuttal/inst/doubleControl_ZREIR25a9r21_0.80.81.4_re.png} & 
        \includegraphics[width=\angles, height=\angles]{figures/rebuttal/inst/outf1.5_1.0_15.0_doubleControl_ZRE25a9r21_0.80.81.4_200_00-160.png} \\
    
        \bottomrule
        \end{tabularx}
    \end{minipage}\hfill
    \begin{minipage}[b]{.49\linewidth}
        \centering
        \caption{Visual comparison with ArtUp [44].}
        \vspace{-5pt}
        \label{tab:angle}
        \centering
        \begin{tabularx}{\linewidth}{>{\centering\arraybackslash}X *{3}{>{\centering\arraybackslash}X}}
    
        \toprule
        Input &  ArtUp & Face2QR \\
        \midrule
    
        \includegraphics[width=\angles, height=\angles]{figures/rebuttal/origin/zre_91.jpg} & 
        \includegraphics[width=\angles, height=\angles]{figures/rebuttal/artup/boy.JPG} & 
        \includegraphics[width=\angles, height=\angles]{figures/rebuttal/gen/9192/outf1.5_1.0_15.0_doubleControl_ZRE91a2r25_0.80.81.4_200_00-100.png} \\
    
        \includegraphics[width=\angles, height=\angles]{figures/rebuttal/origin/zre_92.jpg} & 
        \includegraphics[width=\angles, height=\angles]{figures/rebuttal/artup/man.JPG} & 
        \includegraphics[width=\angles, height=\angles]{figures/rebuttal/gen/9192/outf1.5_1.0_15.0_doubleControl_ZRE92a4r25_0.80.81.4_200_00-80.png} \\
    
        \bottomrule
        \end{tabularx}
    \end{minipage}
    \vspace{-5pt}
\end{table*}

\vspace{-5pt}

\begin{table*}[h]
    \newlength{\mfigwidth}
    \setlength{\mfigwidth}{0.156\textwidth}
    \vspace{-5pt}
    \caption{Real face images of ordinary people (Row 1) collected from [51], generated realistic face (left three on Row 3) using StyleGAN2 [52] and cartoon faces (right three on Row 3) with corresponding QR images $I^o$ (Rows 2 and 4).
    }
    \vspace{-5pt}
    \label{tab:comparison}
    \centering
    \begin{tabularx}{\linewidth}{>{\centering\arraybackslash}X *{5}{>{\centering\arraybackslash}X}}

    \toprule

    \includegraphics[width=\mfigwidth, height=\mfigwidth]{figures/rebuttal/origin/zre_10.jpg} & 
    \includegraphics[width=\mfigwidth, height=\mfigwidth]{figures/rebuttal/origin/zre_2.jpg} &
    \includegraphics[width=\mfigwidth, height=\mfigwidth]{figures/rebuttal/origin/zre_1.jpg} & 
    \includegraphics[width=\mfigwidth, height=\mfigwidth]{figures/rebuttal/origin/zre_16.jpg} & 
    \includegraphics[width=\mfigwidth, height=\mfigwidth]{figures/rebuttal/origin/zre_3.jpg} & 
    \includegraphics[width=\mfigwidth, height=\mfigwidth]{figures/rebuttal/origin/zre_6.jpg} \\

    \includegraphics[width=\mfigwidth, height=\mfigwidth]{figures/rebuttal/gen/5true_faces/outf1.5_1.0_15.0_doubleControl_ZRE10a16r18_0.80.81.4_200_00-100.png} & 
    \includegraphics[width=\mfigwidth, height=\mfigwidth]{figures/rebuttal/gen/5true_faces/outf1.5_1.0_15.0_doubleControl_ZRE2a9r17_0.80.81.4_200_00.png} &
    \includegraphics[width=\mfigwidth, height=\mfigwidth]{figures/rebuttal/gen/5true_faces/outf1.5_1.0_15.0_doubleControl_ZRE1a4r17_0.80.81.4_200_00-120OK.png} & 
    \includegraphics[width=\mfigwidth, height=\mfigwidth]{figures/rebuttal/gen/5true_faces/outf1.5_1.0_15.0_doubleControl_ZRE16a0r18_0.80.81.4_200_00-100.png} & 
    \includegraphics[width=\mfigwidth, height=\mfigwidth]{figures/rebuttal/gen/5true_faces/outf1.5_1.0_15.0_doubleControl_ZRE3a4r17_0.80.81.4_200_00-160.png} & 
    \includegraphics[width=\mfigwidth, height=\mfigwidth]{figures/rebuttal/gen/5true_faces/outf1.5_1.0_15.0_doubleControl_ZRE6a16r17_0.80.81.4_200_00-200.png} \\

    \midrule

    \includegraphics[width=\mfigwidth, height=\mfigwidth]{figures/rebuttal/origin/zre_31.jpg} & 
    % \includegraphics[width=\mfigwidth, height=\mfigwidth]{figures/rebuttal/origin/zre_35.jpg} &
    % \includegraphics[width=\mfigwidth, height=\mfigwidth]{figures/rebuttal/origin/zre_36.jpg} & 
    % \includegraphics[width=\mfigwidth, height=\mfigwidth]{figures/rebuttal/origin/zre_39.jpg} & 
    \includegraphics[width=\mfigwidth, height=\mfigwidth]{figures/rebuttal/origin/zre_42.jpg} &
    \includegraphics[width=\mfigwidth, height=\mfigwidth]{figures/rebuttal/origin/zre_37.jpg} &
    \includegraphics[width=\mfigwidth, height=\mfigwidth]{figures/rebuttal/origin/zre_62.jpg} &
    \includegraphics[width=\mfigwidth, height=\mfigwidth]{figures/rebuttal/origin/zre_54.jpg} &
    \includegraphics[width=\mfigwidth, height=\mfigwidth]{figures/rebuttal/origin/zre_21.jpg} \\

    \includegraphics[width=\mfigwidth, height=\mfigwidth]{figures/rebuttal/gen/5virtual_faces/outf1.5_1.0_15.0_doubleControl_ZRE31a19r22_0.80.81.4_200_00-200.png} & 
    % \includegraphics[width=\mfigwidth, height=\mfigwidth]{figures/rebuttal/gen/5virtual_faces/outf1.5_1.0_15.0_doubleControl_ZRE35a11r22_0.80.81.4_200_00-200.png} &
    % \includegraphics[width=\mfigwidth, height=\mfigwidth]{figures/rebuttal/gen/5virtual_faces/outf1.5_1.0_15.0_doubleControl_ZRE36a6r22_0.80.81.4_200_00-200.png} & 
    % \includegraphics[width=\mfigwidth, height=\mfigwidth]{figures/rebuttal/gen/5virtual_faces/outf1.5_1.0_15.0_doubleControl_ZRE39a4r22_0.80.81.4_200_00-200.png} & 
    \includegraphics[width=\mfigwidth, height=\mfigwidth]{figures/rebuttal/gen/5virtual_faces/outf1.5_1.0_15.0_doubleControl_ZRE42a3r22_0.80.81.4_200_00-200.png} & 
    \includegraphics[width=\mfigwidth, height=\mfigwidth]{figures/rebuttal/gen/5virtual_faces/outf1.5_1.0_15.0_doubleControl_ZRE37a6r22_0.80.81.4_200_00-200.png} &
    \includegraphics[width=\mfigwidth, height=\mfigwidth]{figures/rebuttal/gen/5cartoon_faces/outf1.5_1.0_15.0_doubleControl_ZRE62a11r26_0.80.81.4_200_00-100.png} &
    \includegraphics[width=\mfigwidth, height=\mfigwidth]{figures/rebuttal/gen/5cartoon_faces/outf1.5_1.0_15.0_doubleControl_ZRE54a21r23_0.80.81.4_200_00-200.png} &
    \includegraphics[width=\mfigwidth, height=\mfigwidth]{figures/rebuttal/gen/5cartoon_faces/outf1.5_1.0_15.0_doubleControl_ZRE21a9r18_0.80.81.4_200_00-180.png}
    \\

    \bottomrule
    \end{tabularx}
    \vspace{-5pt}
\end{table*}

\vspace{-5pt}

\begin{table*}[h!]
    \vspace{-5pt}
    \centering
    \newlength{\Blen}
    \setlength{\Blen}{0.156\linewidth}
    \newlength{\Dlen}
    \setlength{\Dlen}{0.156\linewidth}
    \begin{minipage}[b]{.42\linewidth}
    \caption{Bad cases caused by failure of generative model.}
    \vspace{-5pt}
        \label{tab:IDRE}
        \centering
        
        \begin{tabularx}{\linewidth}{>{\centering\arraybackslash}X >{\centering\arraybackslash}X *{1}{>{\centering\arraybackslash}X}}
    
        \toprule
        Input & Output \\ \midrule
        % Input & {Halftone QR~\cite{chu2013halftone}} &  ArtCoder~\cite{su2021artcoder} & Quick QR~\cite{quickqr} & Text2QR (\todo{how to cite}) & Selfie2QR (ours) \\
        % \midrule
    
        \includegraphics[width=\Dlen, height=\Dlen]{figures/rebuttal/origin/zre_32.jpg} & 
        \includegraphics[width=\Dlen, height=\Dlen]{figures/rebuttal/bad/outf1.5_1.0_15.0_doubleControl_ZRE32a7r22_0.80.81.4_200_00-200.png} \\
    
    
        \includegraphics[width=\Dlen, height=\Dlen]{figures/rebuttal/origin/zre_38.jpg} & 
        \includegraphics[width=\Dlen, height=\Dlen]{figures/rebuttal/bad/outf1.5_1.0_15.0_doubleControl_ZRE38a28r22_0.80.81.4_200_00-200.png} \\
    
        \bottomrule
        \end{tabularx}
    \end{minipage}\hfill
    \begin{minipage}[b]{.54\linewidth}
        \caption{Image difference visualization $D$ of uniform loss (first row) and adaptive loss (second row).}
        \vspace{-5pt}
        \label{tab:IDSE}
        \centering
        \begin{tabularx}{\linewidth}{>{\centering\arraybackslash}X *{2}{>{\centering\arraybackslash}X}}
    
        \toprule
        $I^o$ & $D$
        & face region
        \\ \midrule
    
    
        \includegraphics[width=\Blen, height=\Blen]{figures/rebuttal/uniform.png} & 
        \includegraphics[width=\Blen, height=\Blen]{figures/rebuttal/uniformD.png} & 
        \includegraphics[width=\Blen, height=\Blen]{figures/rebuttal/uniformZ.png}  \\

        \includegraphics[width=\Blen, height=\Blen]{figures/rebuttal/adaptive.png} & 
        \includegraphics[width=\Blen, height=\Blen]{figures/rebuttal/adaptiveD.png} & 
        \includegraphics[width=\Blen, height=\Blen]{figures/rebuttal/adaptiveZ.png}  \\
        
        \bottomrule
        \end{tabularx}
    \end{minipage}
    \vspace{-10pt}
\end{table*}
